Benchmarking LLMs for Environmental Review and Permitting

The National Environment Policy Act (NEPA) stands as a foundational piece of environmental legislation in the United States, requiring federal agencies to consider the environmental impacts of their proposed actions. The primary mechanism for achieving this is through the preparation of Environmental Assessments (EAs) and, for significant impacts, comprehensive Environmental Impact Statements (EIS). Large Language Model (LLM)s' effectiveness in specialized domains like NEPA remains untested for adoption in federal decision-making processes. To address this gap, we present NEPA Question and Answering Dataset (NEPAQuAD), the first comprehensive benchmark derived from EIS documents, along with a modular and transparent evaluation pipeline, MAPLE, to assess LLM performance on NEPA-focused regulatory reasoning tasks. Our benchmark leverages actual EIS documents to create diverse question types, ranging from factual to complex problem-solving ones. We built a modular and transparent evaluation pipeline to test both closed- and open-source models in zero-shot or context-driven QA benchmarks. We evaluate five state-of-the-art LLMs using our framework to assess both their prior knowledge and their ability to process NEPA-specific information. The experimental results reveal that all the models consistently achieve their highest performance when provided with the gold passage as context. While comparing the other context-driven approaches for each model, Retrieval Augmented Generation (RAG)-based approaches substantially outperform PDF document contexts, indicating that neither model is well suited for long-context question-answering tasks. Our analysis suggests that NEPA-focused regulatory reasoning tasks pose a significant challenge for LLMs, particularly in terms of understanding the complex semantics and effectively processing the lengthy regulatory documents.

==> figAlgTabs/Figure_3Plots_Docs.tex <==
\begin{figure*}[h]
\centering
\begin{subfigure}{.3\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/3_plots_docs/Sonnet.png}
    \caption{Claude}
\end{subfigure}%
\begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/3_plots_docs/Gemini.png}
    \caption{Gemini}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/3_plots_docs/GPT-4.png}
    \caption{GPT-4}
\end{subfigure}%

\caption[short]{Evaluation on the correlation between the number of tokens for each document and their corresponding correctness over different configurations of context and LLM models}
\label{fig:accuracy:docs}
\end{figure*}

==> figAlgTabs/Figure_3Plots_Parts.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.3\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/3_plots_parts/Sonnet_rag.png}
    \caption{Claude}
\end{subfigure}%
\begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/3_plots_parts/Gemini_rag.png}
    \caption{Gemini}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/3_plots_parts/GPT-4_rag.png}
    \caption{GPT-4}
\end{subfigure}%

\caption[short]{The evaluation results measured by the Answer Correctness scores of each LLM used over different parts with silver passages provided as context
% \critical{We need a similar plot for the PDF context results}
}
\label{fig:accuracy:parts}
\end{figure*}

==> figAlgTabs/Figure_Benchmark_Generation.tex <==
\begin{figure*}[!t]
\centering
    \includegraphics[width=\linewidth]{images/diagrams/Benchmark_Generation.png}
\caption[short]{Steps of Ground-truth benchmark generation for evaluating LLMs over varied contexts for question-answering over EIS documents}
\label{fig:diagram:BenchmarkGeneration}
\end{figure*}

==> figAlgTabs/Figure_Context_Study.tex <==
\begin{figure}
\centering
    \includegraphics[width=\linewidth]{images/diagrams/FlowDiagram.png}
\caption[short]{Illustration of varied contexts we use for comparison with our proposed RAG model for EIS documents.}
\label{fig:diagram:ContextStudy}
\end{figure}

==> figAlgTabs/Figure_RAG_Overview.tex <==
% https://pnnl.sharepoint.com/:u:/r/teams/PolicyAI/_layouts/15/Doc.aspx?sourcedoc=%7B5d719a9f-c940-4459-9043-b662f56292fc%7D&action=edit&or=PrevEdit&cid=606a9e5c-dc23-4780-b2f7-b23dee118b97
\begin{figure*}[ht]
\centering
    \includegraphics[width=\linewidth]{images/diagrams/RAG_Overview-v2.png}
\caption[short]{Architecture overview of RAG solution for building Question-Answering system over EIS Documents}
\label{fig:diagram:RAGOverview}
\end{figure*}

==> figAlgTabs/Listing_AlgorithmCheck.tex <==
\begin{python}[float=*,captionpos=b, basicstyle=\small,caption={Algorithm for Prompt's Response Retrieval with Validation},label={lst:algm:promptValidation}]
function generateResponses(prompt,context,model,max_run_time=10):
    is_success=False;
    index_run_time=1
    while (index<=max_run_time and not is_success):
        csv_object=model.getResponse(prompt,context)
        if isCorrectFormat(csv_object):
            is_success=True;
            break;
        else:
            index_run_time+=1
\end{python}

==> figAlgTabs/Listing_Prompt.tex <==
\begin{lstlisting}[float=*,captionpos=b, basicstyle=\small,caption={Template of prompts for ground-truth benchmark generation},label={lst:prompt:questionGen}]
Can you generate {Number} questions given the content in the following paragraph? 
Restrict the type of generated questions as {Question Type}.
Definition of a "comparison" question: {Question Type Definition} 
You can generate similar questions (but not limited) to sample questions below.
Return in CSV format with three columns: question/ answer/ proof.
Sample questions: {Sample Questions}
Content of the paragraph: {Gold Passage}
\end{lstlisting}

==> figAlgTabs/Table_DatasetStatistics.tex <==
\begin{table*}
\begin{center}

    \setlength\tabcolsep{1pt}
    % \resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|r|r|}
\hline
\multicolumn{1}{|c|}{\textbf{Document Title}}             & \multicolumn{1}{c|}{\textbf{ID}} & \multicolumn{1}{c|}{\textbf{Num. of Pages}} & \multicolumn{1}{c|}{\textbf{Num of Tokens}} \\ \hline
Continental United States Interceptor Site                & CUSIS                            & 74                                          & 41,742                                       \\ \hline
FirstNet                                                  & FN                               & 86                                          & 43,985                                       \\ \hline
Fort Wainwright Alaska                                    & FWA                              & 618                                         & 514,003                                      \\ \hline
Goldrush Mine Project of FEIS in October 2023             & GMP\_FEIS                        & 454                                         & 413,083                                      \\ \hline
Land Management Plan                                      & LMP                              & 472                                         & 325,641                                      \\ \hline
PEIS for Oil and Gas                                      & PEIS\_OG                         & 404                                         & 271,545                                      \\ \hline
Sea Port Oil Terminal                                     & SPOT                             & 890                                         & 613,214                                      \\ \hline
Supplement Analysis of the Final Tank Closure in Richland & SA\_FTC\_R                       & 63                                          & 43,167                                       \\ \hline
T7A Recapitalization                                      & TR                               & 472                                         & 179,697                                      \\ \hline
\end{tabular}
% }
    
\end{center}
\caption{Statistics on the selected EP documents for evaluation}
\label{tbl:dataset:statistics}
\end{table*}

==> figAlgTabs/Table_Human_Evaluator.tex <==
% \begin{table*}[]
% \centering
% \begin{tabular}{|l|ll|ll|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Aspect}}} & \multicolumn{2}{c|}{\textbf{With Experts' Knowledge}}                                     & \multicolumn{2}{c|}{\textbf{Without Experts' Knowledge}}                                         \\ \cline{2-5} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\textbf{Score}} & \multicolumn{1}{c|}{\textbf{Agreement}} & \multicolumn{1}{c|}{\textbf{Score}}   & \multicolumn{1}{c|}{\textbf{Agreement}} \\ \hline
% is\_human\_proof\_correct                              & \multicolumn{1}{l|}{87.50\%}        & \textbf{31.44\%}                        & \multicolumn{1}{l|}{\textbf{95.50\%}} & -3.21\%                                 \\ \hline
% is\_answer\_correct                                    & \multicolumn{1}{l|}{84.00\%}        & \textbf{13.85\%}                        & \multicolumn{1}{l|}{\textbf{87.50\%}} & 13.64\%                                 \\ \hline
% is\_question\_type\_correct                            & \multicolumn{1}{l|}{79.50\%}        & \textbf{84.72\%}                        & \multicolumn{1}{l|}{\textbf{82.00\%}} & 72.97\%                                 \\ \hline
% question\_hard\_level                                  & \multicolumn{1}{l|}{\textbf{2.32}}  & 18.55\%                                 & \multicolumn{1}{l|}{1.98}             & \textbf{33.93\%}                        \\ \hline
% \end{tabular}
% \caption{The scores along with their corresponding human inter annotator agreement scores (Cohen Kappa scores) of different aspects on human evaluation over sampled 100 questions}
% \label{tbl:HumanEvaluator}
% \end{table*}

% \begin{table}[]
% \begin{tabular}{|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Aspect}} & \multicolumn{1}{c|}{\textbf{Original}} & \multicolumn{1}{c|}{\textbf{Augmented}} \\ \hline
% human proof correct             & 93\%                                        & \textbf{87\%}                            \\ \hline
% answer correct                   & 85\%                                        & \textbf{77\%}                            \\ \hline
% question type correct           & 84\%                                        & \textbf{82\%}                            \\ \hline
% \end{tabular}
% \caption{The average scores of human judgement with different aspects  over sampled 100 questions}
% \label{tbl:HumanEvaluator}
% \end{table}

==> figAlgTabs/Table_Question_Distribution.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|l|ll|}
\hline
\multicolumn{1}{|c|}{\textbf{Question Type}} & \multicolumn{2}{c|}{\textbf{Number of questions}}                        \\ \hline
Closed                                       & \multicolumn{1}{l|}{789}           & 49\%                                \\ \hline
Comparison                                   & \multicolumn{1}{l|}{64}            & 4\%                                 \\ \hline
Convergent                                   & \multicolumn{1}{l|}{109}           & 7\%                                 \\ \hline
Divergent                                    & \multicolumn{1}{l|}{121}           & 8\%                                 \\ \hline
Evaluation                                   & \multicolumn{1}{l|}{64}            & 4\%                                 \\ \hline
Funnel                                       & \multicolumn{1}{l|}{127}           & 8\%                                 \\ \hline
Inference                                    & \multicolumn{1}{l|}{101}           & 6\%                                 \\ \hline
Problem-solving                              & \multicolumn{1}{l|}{11}            & 1\%                                 \\ \hline
Process                                      & \multicolumn{1}{l|}{108}           & 7\%                                 \\ \hline
Recall                                       & \multicolumn{1}{l|}{105}           & 7\%                                 \\ \hline
\multicolumn{1}{|c|}{\textbf{Total}}         & \multicolumn{1}{l|}{\textbf{1599}} & \multicolumn{1}{l|}{\textbf{100\%}} \\ \hline
\end{tabular}
\caption{Statistics on Question Types used in our work}
\label{tbl:qt:distribution}
\end{table}

==> sections/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}
\note{need to update this section}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sections/discussion.tex <==
\subsection{Discussion}
\label{sec:discussion}

\paragraph{RAG for Question-Answering Over Domain-Specific Documents}
The findings of this study underscore the significant role of RAG models as crucial strategies for addressing domain-specific questions. These models have shown remarkable superiority in performance compared to zero-shot knowledge and using the full PDF as context. While evaluating LLMs in well-established fields such as mathematics or biology can be straightforward, using numerous human-written sets of ground-truth questions and answers \cite{geminiteam2024gemini}, evaluating domain-specific LLMs necessitates unsupervised or semi-supervised approaches to generate evaluation benchmarks. We recognize that while our approach satisfies the need for an automated method in this domain, it still faces challenges, particularly that the selected question types might not be representative of other research areas. Therefore, researchers in other domains should carefully consider the types of questions they want to generate for their studies.

\paragraph{Patterns of Output} From this study, we draw two overall conclusions regarding the output patterns. First, surprisingly, we did not observe specific patterns of correctness in relation to document metadata such as token counts. This finding contradicts our initial assumption that documents with the lowest token counts would achieve the lowest accuracy and vice versa. We believe one reason for this may be that we selected only 90 passages as gold passages from the document, which might not be representative. Second, we noted that each LLM model tends to have distinctive response types. For instance, Gemini's responses tend to be straightforward when no context is provided, often stating "I don't have the context." In contrast, Claude and GPT-4 are more likely to attempt clarifications of input questions, such as predicting and providing the full content of abbreviations. We encourage researchers in other projects involving RAG to analyze patterns of output to enhance their work.

\ignore{
\paragraph{Static vs Dynamic Models} While using RAG systems, which are based on the Information Retrieval (IR) module and the Generation module, we identified a distinct difference between these two components. While the results from LLMs can change with minor modifications to the questions, the output of the IR, specifically the generation of silver passages, does not significantly change even if we slightly modify the content of the input. Compared to the considerably dynamic generation process, the silver passages extraction is more static. We suggest that future researchers consider two strategies to make the IR part more dynamic. First, they could try and analyze the performance of their models using multiple text embedding engines (besides the BGE used in this work). Second, rather than viewing IR and generation as two separate modules, an integrated approach could be developed that rewards the embedding module after each correct LLM generation and vice versa, to enhance the overall performance of the RAG system.
}
\paragraph{Long Context Reasoning}
One of the primary objectives of this study is to assess how beneficial the long context models that can process 128K to 1.5M tokens context in answering questions from long EIS documents. We noticed that these models struggle to use long input contexts to answer more difficult questions that require multiple steps of reasoning (e.g, problem-solving). Given that we see the model performance varies over the positions and types of questions, we assume that effective question-type and -complexity aware reranking of retrieved documents may help to improve the performance~\cite{jeong2024adaptive}. For example, we can use of another LLM to adjust the order of retrieved chunks based on the problem-solving question type.

\ignore{
\paragraph{Cost vs. Utility}
Given the performance advantages of RAG over long-context LLMs in the NEPA domain, we advocate for increased focus on enhancing RAG, particularly due to the potential cost efficiencies it offers. 
For instance, when a user submits multiple queries regarding a lengthy document to a long-context LLM, each query incurs charges for the same input tokens derived from the PDF. 
However, with RAG, the cost is significantly reduced because it pre-selects relevant passages, thereby reducing the number of input tokens required. 
This is especially advantageous when expanding the LLM products to a larger user base, where cost-effectiveness becomes increasingly critical.
}

==> sections/ethics.tex <==
\section{Ethical Consideration}

It has generally been the norm to assume that previously published work can be used as-is without having to consider the inherited ethical issues. However, in present  times, researchers should not “simply assume that [...] research will have a net positive impact on the world” \cite{hecht2021s}. We acknowledge that this applies not just to new work, but also when using existing work in the way that we have done.

While working on this project, care has been taken to ensure that any and all data was anonymized and no Personally Identifiable Information (PII) is present in the data used. We had domain experts in the team throughout the process, thereby ensuring they were aware of all the potential risks and benefits.

While we do not anticipate the novel work presented here to introduce new ethical concerns in and by themselves, we do recognize that there may also be pre-existing concerns and issues of the data, models, and methodologies we have used for this paper. In particular, it has been seen that LLMs, like the ones used in this work, exhibit a wide variety of bias --  religious, gender, race, profession, and cultural -- and frequently generate answers that are incorrect, misogynistic, antisemitic, and generally toxic~\cite{abid2021persistent,buolamwini2018gender,liang2021towards,nadeem-etal-2021-stereoset,welbl2021challenges}. However, when used within the parameters of our experiments detailed in this paper, we did not see such behaviour from any of the models. To our knowledge, when used as intended, our models do not pose additional ethical concerns than any other LLM.

==> sections/experiments.tex <==
\section{Experimental Setup}
\label{sec:experimental_setup}

% \subsection{Configurations for Response Generation}
% We ran the response generation sequentially on the same Virtual Machine with 64GB of RAM. 
% Each configuration took approximately four hours to generate responses to all the questions.

Our experimental framework is designed to comprehensively evaluate the performance of various \gls*{llm}s in responding to questions related to \gls*{nepa} documents. We selected a diverse set of models, including both closed and open-source options, to provide a broad perspective on current \gls*{llm} capabilities in this domain. The models under evaluation are: GPT-4 (OpenAI)~\cite{openai2024gpt4}, Claude-3 Sonnet (Anthropic)~\cite{ClaudeSonnet}, Gemini (Google)~\cite{geminiteam2024gemini}, 8B LLAMA3.1 (Meta)\cite{dubey2024llama} and 7B Mistral (Mistral AI) \cite{jiang2023mistral}. To assess these models' performance across different scenarios, we developed a benchmark consisting of questions derived from \gls*{nepa} documents. Each model will be evaluated under four distinct context conditions, allowing us to analyze how different levels of information availability affect their responses. The comprehensive evaluation framework will allow us to draw meaningful conclusions about the strengths and limitations of different \gls*{llm}s in handling \gls*{nepa}-related queries under varying levels of contextual information.

\subsection{Context Variation}
\label{sec:contexts}
We designed four distinct context scenarios that simulate various real-world information retrieval situations. These scenarios are designed to test the models' capabilities under different levels of available context:

\noindent\textbf{No Context:} In this baseline scenario, questions are presented to the models without any additional context. While this strategy can work well with popular domains such as sport or literature, we assume that the \gls*{nepa} domain may be challenging for the \gls*{llm}s to provide accurate answers. In other words, this setting can be considered a test of the \gls*{llm}s' ability to answer out-of-general-domain questions. As such, this setting is usually expected to return low performance.

\noindent\textbf{PDF Context:} In this scenario, in addition to the question, we also provide the model with text contents from the entire PDF document, from which the benchmark question was generated. Since we do not inform the model which part of the document to look at, the accuracy of generated responses will heavily depend on the models' ability to pick the correct context from the very large scale textual information provided. We expect this setting to yield performance better than the `no context' scenario. This setup evaluates the models' ability to process and extract relevant information from lengthy, complex documents.

\noindent\textbf{Augmented Context:}~
% \note{is "Augmented Context" a better word choice here?}
Employing a \gls*{rag} approach, this setup provides the top-$k$ most relevant text chunks retrieved from a vector database containing text chunks of \gls*{nepa} documents. In our \gls*{rag} model implementation, when a question is inputted for \gls*{llm} generation, the corresponding context is extracted as a relevant passage from a given \gls*{nepa} document. We use the standard \gls*{rag} setup where we encode both question and retrieved passages with the BGE embedding model~\cite{bge_embedding}. Cosine similarity scores are used to assess the similarity between the question and the contexts. In our case, the number of top-ranked relevant text chunks extracted is set at $k=3$. This scenario assesses the models' performance when given highly relevant, focused information that is specifically retrieved to answer the question at hand.

\noindent\textbf{Gold Context:}~
In this configuration, we include the actual context from which the question was generated in the prompt, alongside the question content. This scenario represents an ideal case where the most relevant information is perfectly identified and provided. hile the situation where users manually identify the correct text passage is rare in practice, we simulate this scenario to measure how well \gls*{llm}s can perform, if we were able to extract relevant passages with very high accuracy. This setup serves as an upper bound for performance, testing the models' ability to comprehend and utilize perfectly relevant information.

\subsection{Evaluation Metrics}
\label{sec:eval_metrics}
To assess the performance of the models across different configurations, we employ a sophisticated evaluation approach that goes beyond simple syntactic similarity measures. While overlap based metrics such as BLEU scores \cite{036_BLEU} have been used in prior works, they are not ideal for evaluations where semantic accuracy is crucial. Therefore, we have chosen to use the RAGAS evaluation framework~\cite{es2023ragas}, specifically focusing on the \textit{answer correctness} score. The \textit{answer correctness} score combines two key aspects -- (i) \textit{factual correctness}: this measures the accuracy of the generated answer at the phrase/clause level compared to the ground truth. We utilize GPT-4 to quantify the factual overlap between the generated answer and the expected answer~\cite{es2023ragas}. (ii) \textit{semantic correctness}: this is calculated by comparing the vector embeddings of the expected answers and the predicted answers using the BGE embedding model~\cite{bge_embedding}. In our evaluation, we assign different weights to these aspects -- $75\%$ for \textit{factual correctness} (weight of 0.75), and $25\%$ for \textit{semantic correctness} (weight of 0.25). This weighting allows us to prioritize factual accuracy while still considering the overall semantic similarity of the responses. By using this comprehensive evaluation metric, we aim to provide a more nuanced and accurate assessment of the \gls*{llm}s' performance in handling \gls*{nepa}-related queries across the different context scenarios. This approach enables us to capture both the precise factual content and the broader semantic accuracy of the generated responses, offering valuable insights into the models' capabilities in processing and utilizing relevant document information.

We employ a separate evaluation method for closed type questions which have only `yes' or `no' answers using the following steps. First, we process the responses generated by the \gls*{llm}s to extract only the `yes' or `no' answer from the generated response. Any additional explanatory text or elaboration is removed from the response. Thereafter, the cleaned binary response is compared directly with the ground truth answer. If the cleaned response exactly matches the ground truth, it is assigned a full score of $100\%$. If there is any discrepancy, including cases where the model fails to provide a clear "Yes" or "No" answer, the response is scored as $0\%$. This straightforward evaluation method for closed questions allows us to assess the models' ability to provide accurate binary responses without being influenced by any uncertainties introduced by the RAGAS evaluation framework. We refer this metric as \textit{answer correctness} score for closed type questions.

==> sections/rag.tex <==
\section{Experimental Setup}

\begin{figure*}[ht]
\centering
    \includegraphics[width=\linewidth]{images/diagrams/RAG_Overview-v2.png}
\caption[short]{Architecture overview of RAG solution for building Question-Answering system over EIS Documents}
\label{fig:diagram:RAGOverview}
\end{figure*}

% \subsection{NEPAQuAD Benchmark}
We describe the processes of our building and evaluating our RAG models for the domain of EIS documents in Figure \ref{fig:diagram:RAGOverview}. 
Before going through each module of RAG models, we describe the construction of the NEPAQuAD ground-truth benchmark that is required for evaluating RAG models as following.

\subsection{NEPAQuAD Benchmark}
Similar to other LLM models \cite{lewis2021retrievalaugmented,munikoti2024atlantic}, our RAG models require a ground-truth benchmark to evaluate the quality of automated responses generated from LLMs, given inputs as questions and a database of passages from an EIS document. Due to the high costs associated with manually creating human-written questions and answers, and the inability to use ground-truth benchmarks from other domains, we adopt a semi-automatic approach to generate the ground-truth benchmark, which we will describe in the next section. Generally, our generated ground-truth benchmark consists of triples containing the following information: a question, an answer, and the proof (i.e., the quotation directly related to the answer, derived from the context in which the question originated).

\subsubsection{Information Retrieval for Silver Passages Extraction}
\textbf{Silver Passages.}  In RAG models, when a question is inputted for LLM generation, the corresponding context is extracted as a predicted relevant passage from a specified EIS document. In the scenario of question-answering for long EIS documents presented in this paper, we have developed models that allow users to pose questions specific to a document. Our models are designed to be easily extendable to answer questions where the responses may come from multiple documents. We refer to these predicted relevant passages as \textbf{silver passages}.

\textbf{Passage Extraction.}  For extracting textual information from an EIS document in PDF format, our module outputs an array of passages, each with its structural information (such as image captions, tables, or plain text) and metadata, including the page number of origin. This task requires an advanced PDF parser to accurately extract information. In our work, we utilize the PyMuPDF\footnote{https://pymupdf.readthedocs.io/en/latest/} package in Python for this purpose.

\textbf{Passage Embedding.} In this module, each passage generated from the previous step serves as the input for a converter. This converter transforms the textual representation of the passage into a vector suitable for computational use. A critical requirement for an effective passage embedding module is that the generated embeddings must capture both the structural and semantic information of the corresponding passage. Vectors produced by a robust passage embedding model for two textually and semantically similar passages should exhibit a high cosine similarity score. For this task, we employ BGE embedding \cite{bge_embedding}.

\textbf{Question Embedding.} Similar to Passage Embedding, we also leveraged BGE embedding for this task. Given questions' content, which are usually in the form of a short sentence, their corresponding vectors were generated for the next steps.

\textbf{Vector Comparison.} In this step, the output vector from the Question Embedding step is used alongside a database of vectors—each representing a passage extracted from the content of a given EIS document. The purpose of this module is to identify the list of passages most relevant to the input query, measured by the similarity between the vector of the question and the vectors of the passages. We use the cosine similarity score to assess this similarity. The number of top-ranked relevant passages extracted, referred to as top-K silver passages, is set at $k=3$.

\subsubsection{Response Generation and Evaluation}
\textbf{Evaluation Prompt.} The input for these steps follows a specific template, which is divided into two parts. The first part involves requesting the LLMs to answer a designated question, while the second part provides the necessary context. In the RAG model, the context is determined by an Information Retrieval process, which retrieves the top-3 silver passages from the corresponding EIS document used in this domain-specific question-answering system.

\textbf{Response Generation.} Based on the output from the evaluation prompt, this step generates a response as the answer for each input question. We utilize three leading LLMs—Claude-Sonnet, Gemini, and GPT-4—for this task. While each of these LLMs imposes a limit on the number of tokens that can be included in a prompt, the maximum allowable tokens are 128,000 for Claude-Sonnet, 1.5 million for Gemini, and 128,000 for GPT-4. This ensures that inputs are within the acceptable range for each model.

\textbf{Response Evaluation.} In this step, the responses generated by the LLMs are compared to the ground-truth answers for the same input questions, provided they are given the expected context. Selecting evaluation metrics remains an open problem in research on LLMs and RAG models, as discussed in \cite{balaguer2024rag}. We utilize the RAGA scoring framework \cite{es2023ragas} to perform this task. The metrics used for this evaluation will be discussed in detail in the next section.

\subsection{Varying Contexts for Question Prompting}
\input{figAlgTabs/Figure_Context_Study}
Getting predicted context as silver passages can offer both advantages and disadvantages for the response generation component of LLMs. One advantage is that the input question can be automatically enriched with contextual information, enhancing the relevance of responses. However, a significant disadvantage is that the accuracy of the response generation module heavily depends on the quality of the predicted context. This dependency poses the risk that our proposed models may perform worse than other strategies for augmenting context in LLM generation. In this work, we explore the performance of LLMs in answering questions with three additional strategies of context augmentation, depicted in Figure \ref{fig:diagram:ContextStudy}.

\textbf{Zero-shot Knowledge.} In this setting, we simulate the scenario of users asking questions in the same way with when they asked questions in general domains. Users only provided the content of question to the LLM model and users had no idea about the context where the questions came from. Users expected the LLM models to automatically find relevant information from their data sets of article domains. While this strategy can work well with popular domains such as sport or literature, we assume that the domain of EIS documents made by NEPA experts are too specific for the LLM models to get the correct context. In the other word, this setting can be considered that it required LLMs to answer out-of-general-domain questions, which usually returned low performance. In this paper, we called this configuration of the context as \textbf{None}.

\textbf{Full PDF as Context.} This scenario of modified context simulates another strategy of users when inputting questions to LLM models in domain-specific document question-answering. While users couldn't find the corresponding context of a question as usually, they would suggest the LLMs to find the context from the whole content of the PDF. Thus, the generated responses' accuracy will heavily depend on the ability of correct context suggestion from large scale textual information provided from the PDF. We assume that the results over this context configuration are low. We called this configuration as \textbf{Full PDF}, or \textbf{PDF}.

\textbf{Gold Passage as Context.} In this configuration, we include the actual context from which the question was generated in the evaluation prompt, alongside the question content. While the scenario where users manually identify the correct passage to enrich the prompt is rare in practice, we simulate this scenario to measure how well LLMs can perform if we were able to extract relevant passages with very high accuracy. We refer to this configuration of context as \textbf{Gold Passage} or simply \textbf{Gold}.
